Surgery and statistics in 3d gravity

We extend the correspondence between universal statistical features of large-$c$ 2d CFTs and surgery methods in pure AdS$_3$ quantum gravity. In particular, we introduce a method that we call RMT surgery, which relates a large class of off-shell partition functions in 3d gravity to the spectral statistics of general CFT observables. We apply this method to construct and compute an off-shell Euclidean wormhole whose boundaries are four-punctured spheres, which captures level repulsion in the high-energy sector of the boundary CFT. Using a similar gluing prescription, we also explore a new class of off-shell torus wormholes with trumpet boundaries, contributing to statistical moments of the density of primary states. Lastly, we demonstrate that surgery methods can be used as an intermediate step towards computing Seifert manifolds directly in 3d gravity.

==> simpler-wick.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Simpler-Wick
% Simpler Wick contractions in LaTeX
% Copyright (C) 2018  Joshua Ellis
%
%
% This work may be distributed and/or modified under the conditions of the LaTeX
% Project Public License, either version 1.3 of this license or (at your option)
% any later version.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Joshua Ellis.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the LaTeX Project Public License for more
% details.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usetikzlibrary{calc}

\pgfkeys{
  /simplerwick/.is family,
  /simplerwick,
  sep/.store in=\swick@sep,
  sep=3pt,
  offset/.store in=\swick@offset,
  offset=1em,
  line width/.store in=\swick@lwidth,
  line width=0.4pt}

% Works just like \@ifnextchar[, except for digits [1-9]
\def\swick@ifnextdigit#1#2{
    \@ifnextchar 1{#1}{
      \@ifnextchar 2{#1}{
        \@ifnextchar 3{#1}{
          \@ifnextchar 4{#1}{
            \@ifnextchar 5{#1}{
              \@ifnextchar 6{#1}{
                \@ifnextchar 7{#1}{
                  \@ifnextchar 8{#1}{
                    \@ifnextchar 9{#1}{#2}}}}}}}}}}

% Convert the digit to its representation as a word
\def\swick@translate#1{%
  \ifcase#1\or
  one\or
  two\or
  three\or
  four\or
  five\or
  six\or
  seven\or
  eight\or
  nine\fi
}

% Keeping track of which contraction is open or closed.
\newif\ifswick@if@one@
\newif\ifswick@if@two@
\newif\ifswick@if@three@
\newif\ifswick@if@four@
\newif\ifswick@if@five@
\newif\ifswick@if@six@
\newif\ifswick@if@seven@
\newif\ifswick@if@eight@
\newif\ifswick@if@nine@

% Shortcut to the ith 'if' variable
\def\swick@settrue@#1{
  \globaldefs=1
  \csname swick@if@\swick@translate{#1}@true\endcsname
  \globaldefs=0}
\def\swick@setfalse@#1{
  \globaldefs=1
  \csname swick@if@\swick@translate{#1}@false\endcsname
  \globaldefs=0}

% Returns true or false based on whether the ith.  Use as:
%
% \if\swick@cond@4
%   <if true>
% \else
%   <if false
% \fi
\def\swick@cond@#1{
  TT\fi
  \csname ifswick@if@\swick@translate{#1}@\endcsname}

% Check if *any* of the ifs is true.
\def\swick@cond@any#1#2{
  \if\swick@cond@1{#1}\else
    \if\swick@cond@2{#1}\else
      \if\swick@cond@3{#1}\else
        \if\swick@cond@4{#1}\else
          \if\swick@cond@5{#1}\else
            \if\swick@cond@6{#1}\else
              \if\swick@cond@7{#1}\else
                \if\swick@cond@8{#1}\else
                  \if\swick@cond@9{#1}\else
                    {#2}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi}

% Set all ifs back to false.
\def\swick@cond@reset{
  \swick@setfalse@1
  \swick@setfalse@2
  \swick@setfalse@3
  \swick@setfalse@4
  \swick@setfalse@5
  \swick@setfalse@6
  \swick@setfalse@7
  \swick@setfalse@8
  \swick@setfalse@9
}

% Do nothing
\def\swick@ignore#1{}

% Delegate to the appropriate subfunction based on the next char:
% - 0: do nothing
% - [1-9]: Open the given contraction
% - anything else: Open contraction 1
\def\swick@smart{
  \@ifnextchar0{
    \swick@ignore
  }{
    \swick@ifnextdigit{
    \swick@smart@
  }{
    \swick@smart@1
  }}}

% Open or close the given contraction.
\def\swick@smart@#1#2{
  \if\swick@cond@#1
    \swick@end#1{#2}
  \else
    \swick@begin#1{#2}
  \fi}
  
% Open a contraction
\def\swick@begin#1#2{
  % swick@max keeps track of the tallest contraction yet.
  \ifnum\swick@max<#1
    \gdef\swick@max{#1}
  \fi
  \swick@settrue@#1
  \tikzexternaldisable
  \labelmathstyle{}
  \tikzpicture[remember picture, baseline=(swick-open#1.base)]
    \node[use as bounding box, inner sep=0pt, outer sep=0pt] (swick-open#1) {$\refmathstyle{} #2$};
  \endtikzpicture
  \tikzexternalenable
}

\def\swick@end#1#2{
  \swick@setfalse@#1
  \tikzexternaldisable
  \labelmathstyle{}
  \tikzpicture[remember picture, baseline=(swick-close#1.base)]
    \node[use as bounding box, inner sep=0pt, outer sep=0pt] (swick-close#1) {$\refmathstyle{} #2$};
  \endtikzpicture
  \tikz[remember picture, overlay]
    \draw[line width=\swick@lwidth] ($(swick-open#1.north) + (0, 3pt)$)
          -- ($(swick-open#1.base) + (0, \swick@offset) + #1*(0, \swick@sep)$) 
          -- ($(swick-close#1.base) + (0, \swick@offset) + #1*(0, \swick@sep)$) 
          -- ($(swick-close#1.north) + (0, 3pt)$);
  \tikzexternalenable}

% Start the \wick environment, checking optional arguments if needed.
\def\wick{
  \@ifnextchar[{
    \wick@
  }{
    \wick@[]
  }}

\def\wick@[#1]#2{
  \ifmmode
    \begingroup
    \pgfkeys{
        simplerwick,
        #1}
    % Define the variables and commands
    \swick@cond@reset
    \gdef\swick@max{0}
    \def\c{\swick@smart}
    % Here is the text
    #2
    % Add a vbox equal to max height
    \dimen0=\swick@sep
    \multiply\dimen0 by \swick@max
    \advance\dimen0 by \swick@offset
    \vbox to \dimen0{}
    % Check that every has been closed
    \swick@cond@any{
      \PackageWarning{simpler-wick}{%
        I have reached the end of \protect\wick\space with some unclosed
        contractions%
      }{}
    }{}
    \endgroup
  \else
    \PackageWarning{simpler-wick}{%
      \protect\wich\space has been called outside a math environment, this will
      be ignore%
    }
  \fi
}

\endinput

% Local Variables:
% TeX-master: "simpler-wick-doc"
% End:
